CATMA: Conformance Analysis Tool For Microservice Applications

The microservice architecture allows developers to divide the core functionality of their software system into multiple smaller services. However, this architectural style also makes it harder for them to debug and assess whether the system's deployment conforms to its implementation. We present CATMA, an automated tool that detects non-conformances between the system's deployment and implementation. It automatically visualizes and generates potential interpretations for the detected discrepancies. Our evaluation of CATMA shows promising results in terms of performance and providing useful insights. CATMA is available at \url{https://cyber-analytics.nl/catma.github.io/}, and a demonstration video is available at \url{https://youtu.be/WKP1hG-TDKc}.

==> known_causes.tex <==
\section{Known Causes of Non-conformance}\label{sec:known_causes}
%\subsection{Literature study - TUHH, DUT provides input}
This section presents a list of known causes for non-conformance collected from the literature. These causes form the basis for the analysis of detected non-conformances.

The work presented in this deliverable focuses on the detection of non-conformances between static and dynamic models.
To develop our approach, we are interested in the causes of such non-conformances.
Knowledge about sources of such differences might help identify their effects.
To this end, we provide an overview of the current state-of-the-art of detection of non-conformances to guide the development of our approach and to serve as a comparator for our work. 
We disregard non-conformances that are based on hardware, e.g., due to non-deterministic behavior because of multi-threading or similar effects.
The presented publications have been collected by combining the findings of two authors’ independent opportunistic searches on Google Scholar.

Whiting and Andrews~\cite{whiting_drift_and_erosion_20} present causes and possible preventions against architectural drift and erosion.
They list three categories for solutions against it, organizational, tools, and processes. 
As Van Gurp and Bosch presented earlier already~\cite{vangurp_design_erosion_02}, it is argued that architectural degradation is unavoidable with time, since the system is adapted to changing requirements.
%A related phenomenon is technical debt, describing a short-term solution that causes problems in the long-term.
Architectural degradation can lead to residue artifacts in code that lead to discrepancies between implementation and the system behavior observed at run-time.
Thus, the system's age is one possible cause of non-conformances, since in the usual software development life-cycle other causes are introduced over time. 

Unreachable/unused code is a well-known code smell that was first mentioned in 2003 by Wake~\cite{wake_refactoring_2004}. This code smell causes code to never be executed during the run-time of the system and could be introduced in the system due to programming errors. Several works~\cite{caivano_spread_2023,effenberger_code_quality_2022,haas_static_analysis_2020} have shown, that this type of code smell is still an issue within the current age of software development. 
It can be a cause for non-conformances since static analysis usually does not regard whether code is executed or it might only be possible to detect this at run-time when deployment effects occur.
Thus, static analysis typically detects system properties in unreachable code, whereas dynamic analysis does not do so because the properties never show any effect.

Waseem et al~\cite{waseem_on_the_nature_2021} conducted an empirical study on five open-source microservice systems to find the most common issues occurring in these types of systems and to understand what are the most common causes for these errors. The authors present a taxonomy that provides a mapping between the known issues and their underlying causes. As our work focuses on microservice applications, the most common causes presented in this work would aid the development of our tool.

The increase in the adoption of microservice applications also leads to an increase in security threats to these systems.  Hannousse et al~\cite{Hannousse2021_securing} presents a list of security threats that are mostly addressed in literature within the field of microservice applications. Microservices communicate with each other via lightweight network protocols through API endpoints. Having these endpoints (unintentionally) left open to the public without any authorization mechanism in place would allow communication to occur that was not intended in the design. Thus it is not irrational to assume that these security threats could aid us in sketching security-related causes for non-conformances detected between design and deployment.
